Direction-Aware Semi-Dense SLAM

To aide simultaneous localization and mapping (SLAM), future perception systems will incorporate forms of scene understanding. In a step towards fully integrated probabilistic geometric scene understanding, localization and mapping we propose the first direction-aware semi-dense SLAM system. It jointly infers the directional Stata Center World (SCW) segmentation and a surfel-based semi-dense map while performing real-time camera tracking. The joint SCW map model connects a scene-wide Bayesian nonparametric Dirichlet Process von-Mises-Fisher mixture model (DP-vMF) prior on surfel orientations with the local surfel locations via a conditional random field (CRF). Camera tracking leverages the SCW segmentation to improve efficiency via guided observation selection. Results demonstrate improved SLAM accuracy and tracking efficiency at state of the art performance.

==> figures/figureIcpConstraints.tex <==
  \begin{figure}
    \centering
    \begin{tikzpicture}
      \node (one) {
        \includegraphics[width=0.26\columnwidth]{./figures/box_1side_cropped.png}
      };
      \node[below = 1ex of one] (cap1) { 2 trans. \& 1 rot.};
      \node[below = -1ex of cap1] {unconstrained};
      \node[right = 0ex of one] (two) {
        \includegraphics[width=0.28\columnwidth]{./figures/box_2side_cropped.png}
      };
      \node (cap2) at (cap1-|two) { 1 trans.};
      \node[below = -1ex of cap2] {unconstrained};
      \node[right = 0ex of two] (three) {
        \includegraphics[width=0.28\columnwidth]{./figures/box_3side_cropped.png}
      };
      \node at (cap1-|three){fully constrained};
    \end{tikzpicture}
    \caption[Point-to-plane ICP constraints]{Intuition about
    constraints on the point-to-plane ICP cost function depending on the geometry of the map.
   \label{fig:icpConstraints}}
\end{figure}


==> gibbsSampler.tex <==

\begin{algorithm}
  \caption[Gibbs-sampling for joint map and directional segmentation inference]{%
      Gibbs-sampling algorithm for joint inference over surfel-based
      map and directional segmentation. \label{alg:gibbsSparseFusion}}
  \begin{algorithmic}[1]
    \While{more samples desired}
      \State Update set of surfels, neighborhoods, and surfel observations
      \State Sample $n_i \sim p(n_i \mid p_i, p_{\neigh_i}, \mu_{z_i}, \tau_{z_i}, \{x^n_j\}_{j\in O_i})$ (Eq.~\eqref{eq:dirSLAMnormalPost})
      \State Sample $z_i \sim p(z_i \mid n_i, \mu, \tau; \alpha)$ (Eq.~\eqref{eq:labelPosteriorDPvMF})
      \State Sample $\mu_k, \tau_k \sim p(\mu_k, \tau_k \mid n, z, \mu_0, a,b)$ (Eq.~\eqref{eq:dirSLAMdpParamsPost})
      \State Sample $p_i \sim p(p_i \mid n_i, p_{N_i}, z_i, z_{N_i})$ (Eq.~\eqref{eq:dirSLAMposPost})
      \State Update ML estimates $\hat p_i$ and $\hat n_i$ for camera tracking
      \State Update other estimates such as covariance estimates and entropy
    \EndWhile
  \end{algorithmic}
\end{algorithm}


==> notUsing.tex <==

\subsubsection{MAP over map quantities}

For efficiency reasons we choose to find the maximum a-posteriori
estimate for each variable using gradient descent on the negative log
posterior. The resulting cost function to be minimized takes the form
\begin{align}
  f_i(p_i) &= \tfrac{1}{2}\|p_i - p_{i0}\|^2_{\Sigma_0} 
     +\tfrac{1}{2}\sum_{j\in O_i} \| n_i^T(x^p_j - p_i)\|_2^2 
   + \tfrac{1}{2}\sum_{j\in N_i} \Ind{z_i=z_j} \|n_i^T (p_j - p_i)\|_2^2 
\end{align}
The gradient is
\begin{align}
  \deriv{}{p_i} f_i(p_i) &= \Sigma_0^{-1} (p_i - p_{i0}) - \sum_{j\in O_i} 
  n_i^T(x^p_j - p_i) n_i - \sum_{j\in N_i} \Ind{z_i=z_j} n_i^T (p_j - p_i) n_i 
\end{align}

We re-write the gradient to reveal how sufficient statistics of the
data can be used in its computation. 
This is important as it allows
forgetting the individual observations after they have been added to
the sufficient statistics.
We keep track of the following statistic for each surfel:
\begin{align}
  \xSum{x}^p_i &= \sum_{j\in O_i} x^p_j &
  N_i &= | O_i | \,.
\end{align}
With this the term in the gradient involving observations becomes
\begin{align}
   \sum_{j\in O_i} n_i^T(x^p_j - p_i) n_i &= n_i^T(\xSum{x}^p_i - |O_i| p_i) n_i  \,.
\end{align}



\subsubsection{MRF with mean field inference}
%http://www.vision.is.tohoku.ac.jp/files/5713/7139/9160/62-Saito-CVPR12.pdf
Choose mean field since it is easier parallelized.

The joint energy is
\begin{align}
  P(p, x) \propto \exp E(p,x) &= -\tfrac{1}{2}\sum_i\sum_{j\in N_i} \Ind{z_i=z_j} \|\mu_{z_i}^T (p_i - p_j )\|_2^2 
    - \tfrac{1}{2}\sum_{j\in O_i} \| x^p_j - p_i\|^2_{\Sigma_O} 
\end{align}
Assume Gaussian marginal distributions for each point
\begin{align}
  q(p_i) = \GAUSS(p_i; \tilde\mu, \tilde\Sigma)
\end{align}
and thus the approximate joint density is
\begin{align}
  Q(p)  =\prod_i q(p_i)
\end{align}
Variational inference then seeks to minimize 
\begin{align}
  L(Q) &= - \int_p Q(p) \log Q(p) + \int_p Q(p) \log P(p)\\
       &= - \int_p Q(p) \log Q(p) + \int_p Q(p) E(p) \\
       &= - \int_p \prod_i q(p_i) \sum_i \log q(p_i) + \int_{p_{-i}} Q(p)_{p_{-i}} \int_{p_i} q(p_i) E(p) \\
       &= \sum_i H(q_i) + \int_p Q(p) E(p) \\
\end{align}

\begin{align}
  \log q_i^\star &= \ExpectOver{-i}{ \log p( p, x ) } + C= \ExpectOver{-i}{ E( p, x ) } +C \\
           &= \ExpectOver{-i}{
           \sum_i\sum_{j\in N_i} \Ind{z_i=z_j} \|\mu_{z_i}^T (p_i - p_j )\|_2^2 
         + \sum_{j\in O_i} \log \GAUSS (x^p_j; p_i, \Sigma_O) } + C \\
           &= \sum_i\sum_{j\in N_i} 
           \ExpectOver{-i}{\Ind{z_i=z_j} \|\mu_{z_i}^T (p_i - p_j )\|_2^2 }
         + \sum_{j\in O_i} 
            \ExpectOver{-i}{\log \GAUSS (x^p_j; p_i, \Sigma_O) } \\
           &= \sum_i\sum_{j\in N_i} 
           \ExpectOver{-i}{\Ind{z_i=z_j} \|\mu_{z_i}^T (p_i - p_j )\|_2^2 }
         + \sum_{j\in O_i} \log \GAUSS (x^p_j; p_i, \Sigma_O) \\
\end{align}

focusing on the following assuming (for now fixed $\mu_{z_i} = n_i$
\begin{align}
  &\sum_i\sum_{j\in N_i} \ExpectOver{-i}{\Ind{z_i=z_j} \|n_i^T (p_i - p_j )\|_2^2 }\\
  &= C+ \sum_{j\in N_i} \ExpectOver{-i}{\Ind{z_i=z_j} (p_i - p_j )^T n_i^T n_i (p_i-p_j) }\\
  &= C+ \sum_{j\in N_i} \ExpectOver{-i}{\Ind{z_i=z_j} (p_i^T n_i^T n_i p_i -2 p_j^Tn_i^T n_i p_i + p_j^T n_i^T n_i p_j) }
\end{align}


\subsubsection{Mean field Variational inference as implemented and working}
%https://www.cs.princeton.edu/courses/archive/fall11/cos597C/lectures/variational-inference-i.pdf

Assume each point distribution is Gaussian
\begin{align}
  \prod_i \GAUSS(p_i; \mu_i', \Sigma_i') = \prod_i q(p_i)
\end{align}

ELBO
\begin{align}
  L &= \ExpectOver{q}{\log p(\{p_i\}, \{\{x^p_j\}_{O_i}\})} - \ExpectOver{q}{\log q(\{p_i\})} \\
    &= \ExpectOver{q}{\log p(\{p_i\}, \{\{x^p_j\}_{O_i}\})} -\sum_i \ExpectOver{q_i}{\log q_i(p_i)} \\
    &= \log p (\{\{x^p_j\}_{O_i}\}) + \sum_i \ExpectOver{q_i}{\log p(p_i \mid p_{N_i}, \{x^p_j\}_{O_i})} - \ExpectOver{q_i}{\log q_i(p_i)} \\
\end{align}

where the entropy of the mean field distributions is the one of a multi-variate Gaussian
\begin{align}
  \ExpectOver{q_i}{\log q_i(p_i)} = \tfrac{3}{2} \log(2\pi e) + \tfrac{1}{2} \log |\Sigma_i'|
\end{align}

The conditional expectation needed for the parameter update is:
\begin{align}
  &\ExpectOver{\setminus i}{\log p(p_i \mid p_{\setminus i}, \{x^p_j\}_{O_i})} 
  = \ExpectOver{N_i}{\log p(p_i \mid p_{N_i}, \{x^p_j\}_{O_i})}  \\
  &= \ExpectOver{N_i}{\log \prod_{j\in N_i} 
    \GAUSS(p_i; p_j, (n_{i} n_{i}^T)^{-1})^{\Ind{z_i=z_j} }
    \GAUSS(x^p_0; p_i, \Sigma_O) \prod_{j\in O_i} \GAUSS(x^p_j; p_i, (n_i n_i^T)^{-1}) 
    } \\
  &= \ExpectOver{N_i}{\sum_{j\in N_i} 
    \Ind{z_i=z_j} \log \GAUSS(p_i; p_j, (n_{i} n_{i}^T)^{-1})
    + \log \GAUSS(x^p_0; p_i, \Sigma_O)
    + \sum_{j\in O_i} \log \GAUSS(x^p_j; p_i, (n_i n_i^T)^{-1}) 
    } \\
  &= \sum_{j\in N_i}\Ind{z_i=z_j} \ExpectOver{j}{ \log \GAUSS(p_i; p_j, (n_{i} n_{i}^T)^{-1})} 
  + \log \GAUSS(x^p_0; p_i, \Sigma_O) 
    + \sum_{j\in O_i} \log \GAUSS(x^p_j; p_i, (n_i n_i^T)^{-1})
\end{align}
where
\begin{align}
  \sum_{j\in N_i}\Ind{z_i=z_j} &\ExpectOver{j}{ \log \GAUSS(p_i; p_j, (n_{i} n_{i}^T)^{-1})} -\log Z
  = \sum_{j\in N_i}\Ind{z_i=z_j} \ExpectOver{j}{(p_j-p_i)^T n_i  n_i^T (p_j-p_i)  }  -\log Z\\
  &= \sum_{j\in N_i}\Ind{z_i=z_j} \ExpectOver{j}{p_j^T n_i  n_i^T p_j -2 p_j^T n_i  n_i^T p_i + p_i^T n_i  n_i^T p_i}  -\log Z\\
  &= \sum_{j\in N_i}\Ind{z_i=z_j} \ExpectOver{j}{p_j^T n_i  n_i^T p_j} 
  -2 \ExpectOver{j}{ p_j^T} n_i  n_i^T p_i + p_i^T n_i  n_i^T p_i  -\log Z\\
  &= \sum_{j\in N_i}\Ind{z_i=z_j} n_i^T \Sigma_j' n_i+ n_i^T \mu_j' \mu_j'^T n_i 
  -2 \mu_j'^T n_i  n_i^T p_i + p_i^T n_i  n_i^T p_i  -\log Z\\
\end{align}
where
\begin{align}
  \ExpectOver{j}{p_j^T n_in_i^T  p_j } 
  &= \ExpectOver{j}{\tr (p_j^T n_in_i^T  p_j ) }  
  = \ExpectOver{j}{\tr (n_in_i^T  p_j p_j^T ) }  \\
  &= \tr (\ExpectOver{j}{n_in_i^T  p_j p_j^T}  )  
  = \tr (n_in_i^T \ExpectOver{j}{ p_j p_j^T}  )  \\
  &= \tr (n_in_i^T (\Var{p_j} + \ExpectOver{j}{ p_j} \ExpectOver{j}{ p_j^T} ) )  \\
  &= n_i^T \Var{p_j} n_i+ n_i^T \ExpectOver{j}{ p_j} \ExpectOver{j}{ p_j^T} n_i  \\
  &= n_i^T \Sigma_j' n_i+ n_i^T \mu_j' \mu_j'^T n_i  \\
  \ExpectOver{j}{p_j} &= \mu'
\end{align}

\begin{align}
  \log \GAUSS(x^p_0; p_i, \Sigma_O)
  &= (x^p_0 - p_i)^T \Sigma_O^{-1} (x^p_0 - p_i) - \log Z \\
  &= x^{pT}_0 \Sigma_O^{-1} x^p_0 - 2p_i^T \Sigma_O^{-1} x^p_0 + p_i^T \Sigma_O^{-1} p_i - \log Z 
\end{align}
\begin{align}
  \sum_{j\in O_i} \ExpectOver{j}{\log \GAUSS(x^p_j; p_i, (n_i n_i^T)^{-1}) }
\end{align}

Since all terms have the form of Gaussians, the resulting log
distribution is proportional to the product of those Gaussians which
turns out to be a Gaussian as well with the following mean and
covariance:
\begin{align}
  \left(\Sigma'^\star \right)^{-1} 
  &= n_i n_i^T \left(\sum_{j\in N_i} \Ind{z_i=z_j} +\sum_{j\in O_i} \sigma^{-2}_{p,j} \right) + \Sigma_O^{-1} \\
  \mu'^\star &= \Sigma'^\star \left(
    \Sigma_O^{-1} x^p_0
  + \sum_{j\in N_i} \Ind{z_i=z_j} n_i n_i^T \mu_j' 
  + \sum_{j\in O_i} n_i n_i^T x^p_j \sigma^{-2}_{p,j} 
  \right) \\
             &= \Sigma'^\star \left(
    \Sigma_O^{-1} x^p_0
  + n_i n_i^T \left(\sum_{j\in N_i} \Ind{z_i=z_j} \mu_j' 
  + \sum_{j\in O_i}x^p_j \sigma^{-2}_{p,j} \right)
  \right)
\end{align}
where $\sigma_{p,j}$ is the in-plane measurement std of measurement $j$.

\TODO{should probably use $\GAUSS(p_i ; p_j, (n_j n_j^T)_{-1})$ i.e. project onto $n_j$ then:
\begin{align}
  \left(\Sigma'^\star \right)^{-1} 
  &= \sum_{j\in N_i} \Ind{z_i=z_j} n_j n_j^T 
  + n_i n_i^T\sum_{j\in O_i} \sigma^{-2}_{p,j} 
  + \Sigma_O^{-1} \\
  \mu'^\star &= \Sigma'^\star \left(
    \Sigma_O^{-1} x^p_0
  + \sum_{j\in N_i} \Ind{z_i=z_j} n_j n_j^T \mu_j' 
  + n_i n_i^T \sum_{j\in O_i} x^p_j \sigma^{-2}_{p,j} 
  \right) 
\end{align}
works
}

\TODO{to debug try without MRF:
\begin{align}
  \left(\Sigma'^\star \right)^{-1} 
  &= 
    n_i n_i^T\sum_{j\in O_i} \sigma^{-2}_{p,j} 
  + \Sigma_O^{-1} \\
  \mu'^\star &= \Sigma'^\star \left(
    \Sigma_O^{-1} x^p_0
  + n_i n_i^T \sum_{j\in O_i} x^p_j \sigma^{-2}_{p,j} 
  \right) 
\end{align}
did work
}

\TODO{to debug try without MRF and with full observations
\begin{align}
  \left(\Sigma'^\star \right)^{-1} 
  &= \sum_{j\in O_i} \Sigma^{-1}_{p,j} 
  + \Sigma_O^{-1} \\
  \mu'^\star &= \Sigma'^\star \left(
    \Sigma_O^{-1} x^p_0
  + \sum_{j\in O_i} \Sigma^{-1}_{p,j} x^p_j
  \right) 
\end{align}
Dont forget to transform everything into the world coordinates.
that works now and I should use full observations; I had to inflate the
covariance matrix to get (numeric?) stability.

full observations are definitely the way to go
}

to debug try with MRF and with full observations and expectation over $n_i n_i^T$
\begin{align}
  \left(\Sigma'^\star \right)^{-1} 
  &= \Sigma_O^{-1}
  + \sum_{j\in O_i} \Sigma^{-1}_{p,j} 
  + \sum_{j\in N_i} \Expectation{\Ind{z_i=z_j}} \Expectation{n_j n_j^T}  \\
  \mu'^\star &= \Sigma'^\star \left(
    \Sigma_O^{-1} x^p_0
  + \sum_{j\in O_i} \Sigma^{-1}_{p,j} x^p_j
  + \sum_{j\in N_i} \Expectation{\Ind{z_i=z_j}} \Expectation{n_j n_j^T} \mu_j' 
  \right) 
\end{align}
using the expectation over $n_in_i^T$ helped make it work as far as I
can see; sampling is a cleaner story though.


==> sparseFusion.tex <==


